Capacity Planning in Stable Matching

Motivated by the shortage of seats that the Chilean school choice system is facing, we introduce the problem of jointly increasing school capacities and finding a student-optimal assignment in the expanded market. Due to the theoretical and practical complexity of the problem, we provide a comprehensive set of tools to solve the problem, including different mathematical programming formulations, a cutting plane algorithm, and two heuristics that allow obtaining near-optimal solutions quickly. On the theoretical side, we show the correctness of our formulations, different properties of the objective and feasible region that facilitate computation, and also several properties of the underlying mechanism to find a student-optimal matching under capacity expansions. On the computational side, we use data from the Chilean school choice system to demonstrate the impact of our framework and derive insights that could help alleviate the problem. Our results show that each additional seat can benefit multiple students and that we can effectively target the assignment of previously unassigned students or improve the assignment of several students through improvement chains. Nevertheless, our results show that the marginal effect of each additional seat is decreasing and that simply adding seats is insufficient to ensure every student gets assigned to some school. Finally, we discuss several extensions of our framework, showcasing its flexibility to accommodate different needs.

==> plots/L_constraint.tex <==
% \documentclass{article}
% \usepackage{tikz}
% \usepackage{caption}
%  \usepackage{subcaption}
%  \usetikzlibrary{calc}
%  \usepackage{xcolor}

%  \begin{document}

\definecolor{royalblue}{rgb}{0.255, 0.412, 0.882}
\definecolor{canaryyellow}{rgb}{1, 0.937, 0.0}
\definecolor{darkyellow}{rgb}{0.8, 0.8, 0.0}
\begin{figure}[h!]
        \centering
        \begin{tikzpicture}[node distance=2cm, auto]

        % Define the style for the nodes
        \tikzstyle{state}=[rectangle, draw, fill=gray!5, 
            text centered, minimum height=1em, minimum width=1em,font=\fontsize{7}{8}\selectfont]

        % Define the nodes
        \node[state] (v1) {$(s'_5,c)$};
        \node[state] (v2) [right of=v1] { $(s,c)$};
        \node[state] (v3) [right of=v2] {$(s'_4,c)$};
        \node[state] (v4) [right of=v3] {$(s'_3,c)$};
        \node[state] (v5) [right of=v4] {$(s'_2,c)$};
        \node[state] (v6) [right of=v5] {$(s'_1,c)$};

        \node[state] (v7) [above of=v2] {$(s,c'_2)$};
        \node[state] (v8) [above of=v4] {$(s'_3,c'_2)$};
        \node[state] (v9) [above of=v5] {$(s'_2,c'_2)$};
        \node[state] (v10) [above of=v8] {$(s'_3,c'_1)$};
        \node[state] (v11) [above of=v7] {$(s,c'_1)$};
        \node[state] (v12) [right of=v11] {$(s'_4,c'_2)$};

        % \node (l1) [left of=v7] {\hspace{-3cm}\tiny$q_c\cdot \big( 1-{\color{darkyellow}\displaystyle\sum_{c' \succeq c}x_{s,c'}} \big) \leq \color{red}\displaystyle \sum_{s' \succ s}x_{s',c}$};

         % Draw the edges
        \draw[->] (v1) -- (v2);
        \draw[->] (v2) -- (v3);
        \draw[->] (v3) -- (v4);
        \draw[->] (v4) -- (v5);
        \draw[->] (v5) -- (v6);
        \draw[->] (v2) -- (v7);
        \draw[->] (v7) -- (v11);
        \draw[->, bend left] (v4) to (v10);
        \draw[->] (v10) -- (v8);
        \draw[->] (v5) -- (v9);
        \draw[->] (v3) -- (v12);

        % Draw the dashed ellipse around v2, v7, and v10
        \fill[canaryyellow, rounded corners, opacity=0.1]
        ($(v2) + (-0.5, -0.5)$) -- ($(v7) + (-0.5, 0.5)$) -- ($(v11) + (-0.5, 0.5)$) -- ($(v11) + (0.5, 0.5)$) -- ($(v2) + (0.5, -0.5)$) -- cycle;
        \draw[dashed, line width=1.5pt, canaryyellow, rounded corners]
        ($(v2) + (-0.5, -0.5)$) -- ($(v7) + (-0.5, 0.5)$) -- ($(v11) + (-0.5, 0.5)$) -- ($(v11) + (0.5, 0.5)$) -- ($(v2) + (0.5, -0.5)$) -- cycle;
        \fill[red, rounded corners, opacity=0.1]
        ($(v3) + (-0.5, -0.5)$) -- ($(v6) + (0.5, -0.5)$) -- ($(v6) + (0.5, 0.5)$) -- ($(v3) + (-0.5, 0.5)$) -- cycle;
        \draw[dashed, line width=1.5pt, red, rounded corners]
        ($(v3) + (-0.5, -0.5)$) -- ($(v6) + (0.5, -0.5)$) -- ($(v6) + (0.5, 0.5)$) -- ($(v3) + (-0.5, 0.5)$) -- cycle;

        \end{tikzpicture}
    \caption{Example of $L$-constraint for the pair $(s,c) \in \mathcal{E}$. %where school $c$ has capacity 3, and the preference lists are as follows: $c: s'_1,s'_2,s'_3,s'_4,s,s'_5$; $s'_1: c$; $s'_2: c'_2, c$; $s'_3:  c'_2, c'_1, c$; $s'_4:  c'_2, c$; $s: c'_1, c'_2, c$ and $s'_5: c$.
    The yellow area corresponds to $\sum_{c' \succeq c}x_{s,c'}$ while the red represents $\sum_{s' \succ s}x_{s',c}$ in \eqref{eq:L_constraints}.
    }
\label{fig:L_constraint_example}
\end{figure}

 % \end{document}


==> plots/comb_constraint.tex <==
% \documentclass{article}
% \usepackage{tikz}
% \usepackage{caption}
% \usepackage{subcaption}
% \usetikzlibrary{calc}
% \usepackage{xcolor}

% \begin{document}

\definecolor{royalblue}{rgb}{0.255, 0.412, 0.882}
\definecolor{canaryyellow}{rgb}{1, 0.937, 0.0}
\definecolor{darkyellow}{rgb}{0.8, 0.8, 0.0}
\begin{figure}[h!]
    \centering
        \begin{tikzpicture}[node distance=2cm, auto]

        % Define the style for the nodes
        \tikzstyle{state}=[rectangle, draw, fill=gray!5, 
            text centered, minimum height=1em, minimum width=1em,font=\fontsize{7}{8}\selectfont]

        % Define the nodes
        \node[state] (v1) {$(s'_5,c)$};
        \node[state] (v2) [right of=v1] { $(s,c)$};
        \node[state] (v3) [right of=v2] {$(s'_4,c)$};
        \node[state] (v4) [right of=v3] {$(s'_3,c)$};
        \node[state] (v5) [right of=v4] {$(s'_2,c)$};
        \node[state] (v6) [right of=v5] {$(s'_1,c)$};

        \node[state] (v7) [above of=v2] {$(s,c'_2)$};
        \node[state] (v8) [above of=v4] {$(s'_3,c'_2)$};
        \node[state] (v9) [above of=v5] {$(s'_2,c'_2)$};
        \node[state] (v10) [above of=v8] {$(s'_3,c'_1)$};
        \node[state] (v11) [above of=v7] {$(s,c'_1)$};
        \node[state] (v12) [right of=v11] {$(s'_4,c'_2)$};

        %\node (comb1) [left of=v7] {\hspace{-2cm}\tiny ${\color{royalblue}\displaystyle \sum_{(s,c) \in \text{comb}}x_{s,c}}
        %\geq \displaystyle q_c$};

        % Draw the edges
        \draw[->] (v1) -- (v2);
        \draw[->] (v2) -- (v3);
        \draw[->] (v3) -- (v4);
        \draw[->] (v4) -- (v5);
        \draw[->] (v5) -- (v6);
        \draw[->] (v2) -- (v7);
        \draw[->] (v7) -- (v11);
        \draw[->, bend left] (v4) to (v10);
        \draw[->] (v10) -- (v8);
        \draw[->] (v5) -- (v9);
        \draw[->] (v3) -- (v12);

        % Draw the dashed ellipse around v2, v7, and v10
        \fill[royalblue, rounded corners, opacity=0.1] 
            ($(v2) + (-0.5, -0.5)$) -- ($(v7) + (-0.5, 0.5)$) -- ($(v11) + (-0.5, 0.5)$) -- ($(v11) + (0.5, 0.5)$) -- ($(v2) + (0.5, 0.5)$) -- ($(v4) + (-0.5, 0.5)$) -- ($(v10) + (-0.5, 0.5)$) -- ($(v10) + (0.5, 0.5)$) -- ($(v4) + (0.5, 0.5)$) -- ($(v5) + (-0.5, 0.5)$) -- ($(v9) + (-0.5, 0.5)$) -- ($(v9) + (0.5, 0.5)$) -- ($(v5) + (0.5, 0.5)$) -- ($(v6) + (-0.5, 0.5)$) -- ($(v6) + (0.5, 0.5)$) -- ($(v6) + (0.5, -0.5)$) --cycle;
        \draw[dashed, line width=1.5pt, royalblue, rounded corners] 
            ($(v2) + (-0.5, -0.5)$) -- ($(v7) + (-0.5, 0.5)$) -- ($(v11) + (-0.5, 0.5)$) -- ($(v11) + (0.5, 0.5)$) -- ($(v2) + (0.5, 0.5)$) -- ($(v4) + (-0.5, 0.5)$) -- ($(v10) + (-0.5, 0.5)$) -- ($(v10) + (0.5, 0.5)$) -- ($(v4) + (0.5, 0.5)$) -- ($(v5) + (-0.5, 0.5)$) -- ($(v9) + (-0.5, 0.5)$) -- ($(v9) + (0.5, 0.5)$) -- ($(v5) + (0.5, 0.5)$) -- ($(v6) + (-0.5, 0.5)$) -- ($(v6) + (0.5, 0.5)$) -- ($(v6) + (0.5, -0.5)$) --cycle;



        \end{tikzpicture}
        %\caption{The subscripts of $\mathbf{x}$ involved in a comb constraint with base $(s,c)$ (there is more than one).}
 \caption{Example of a comb based on the pair $(s,c) \in \mathcal{E}$ when school $c$ has capacity 3.%, and the preference lists are as follows: $c: s'_1,s'_2,s'_3,s'_4,s,s'_5$; $s'_1: c$; $s'_2: c'_2, c$; $s'_3:  c'_2, c'_1, c$;  $s'_4:  c'_2, c$; $s: c'_1, c'_2, c$ and $s'_5: c$.}
}
\label{fig:comb_constraint}
\end{figure}

% \end{document}

